FIST: A Feature-Importance Sampling and Tree-Based Method for Automatic Design Flow Parameter Tuning

Design flow parameters are of utmost importance to chip design quality and require a painfully long time to evaluate their effects. In reality, flow parameter tuning is usually performed manually based on designers' experience in an ad hoc manner. In this work, we introduce a machine learning-based automatic parameter tuning methodology that aims to find the best design quality with a limited number of trials. Instead of merely plugging in machine learning engines, we develop clustering and approximate sampling techniques for improving tuning efficiency. The feature extraction in this method can reuse knowledge from prior designs. Furthermore, we leverage a state-of-the-art XGBoost model and propose a novel dynamic tree technique to overcome overfitting. Experimental results on benchmark circuits show that our approach achieves 25% improvement in design quality or 37% reduction in sampling cost compared to random forest method, which is the kernel of a highly cited previous work. Our approach is further validated on two industrial designs. By sampling less than 0.02% of possible parameter sets, it reduces area by 1.83% and 1.43% compared to the best solutions hand-tuned by experienced designers.

==> _txt/1_related.tex <==

\section{Related Work}
Space exploration solutions have been performed at various level of abstractions. There exist many studies about design space exploration (DSE) for high-level synthesis. 
For example, genetic algorithms \cite{deb2002fast}\cite{tiwary2006generation} have been utilized in DSE, but requires many trial synthesis jobs \cite{liu2015supervised}. 
Machine learning-based frameworks are also widely adopted~\cite{zuluaga2012smart,zuluaga2013active,mariani2012oscar}. Liu et al. \cite{liu2013learning} further improve the framework by applying tree-based learning model and transductive experimental design (TED) sampling method \cite{yu2006active}. 
Other related machine learning works that exploring co-processor synthesis include \cite{xydis2013meta}\cite{xydis2015spirit}.

FIST learns feature importance from already explored designs. 
We note that some recent works about space exploration have started to transfer prior knowledge. 
For example, \cite{papamichael2015nautilus} improves genetic algorithm by guiding DSE with the expertise from IP authors. 
\cite{li2016efficient} borrows the knowledge from known programs on processor simulators. Compared to FIST, the former requires human knowledge and the latter is actually transferring models to new programs through transfer learning instead of the already explored designs. 
Neither of them targets synthesis space exploration.

==> _txt/5_discussion.tex <==
%=======================================%
%           discussion          %
%=======================================%

\section{Discussion}
 
%\subsection{Sampling by Clustering}
%\begin{table}[!thb]
\begin{table}[!b]
  \centering
  \caption{Ground-truth rank of feature by importance.}
  \label{tbl:t2}
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{c | c| c |c}
  \hline
  Design   & Power   & SetTime & HoldTime   \\
  \hline
  b11        & 2  1  4  5  3  8  9  7 10  6  &  2  1  4  5  3  9  7  8 10  6 &  2  1  4  5  3  8  9  7 10  6  \\
  b12        & 2  1  4  5  8  3  7  9  6 10  &  2  1  5  4  8  9  3 10  6  7 &  2  4  5  1  3  8  9 10  7  6     \\
  b13        & 2  4  5  3  8  1  9  7 10  6  &  2  3  5  1  8  4 10  7  9  6 &  2  1  5  3  4  8  9  7 10  6   \\
  b14        &  2  1  4  3  5  8 10  6  9  7  &  2  1  5  4  3  6 10  9  8  7 &  2  1  5 10  9  3  8  4  6  7     \\
  b15        &   2  1  5  4  3  8 10  7  9  6  & 2  1  5  4  9  8  3 10  6  7 &  2  1  9  5 10  4  3  7  8  6     \\
  b17        &  2  1  4  3  5  8  9  7 10  6  &  2  1  4  6  7  8  3  5  9 10 & 2  1  4  6  8  7  3  5  9 10      \\
  b20        &  2  1  5  4  3  8  6 10  7  9  &  2  1 10  8  9  4  5  3  6  7 & 2  1  9 10  8  3  4  7  6  5     \\
  b21        &  2  1  5  4  3  8  6 10  7  9  &  2  1 10  9  4  8  5  3  6  7 &  2  1  9 10  8  3  4  7  5  6    \\
  b22        &  2  1  4  5  3  8 10  6  7  9  &  2  1  8  4  9 10  3  5  7  6 &  2  1  8 10  9  3  4  5  6  7   \\
  \hline
  \end{tabular}
  }
\end{table}


To further understand the effect of sampling by clustering, both feature importance and sampling result are analyzed. Table \ref{tbl:t2} shows the rank of importance $I$ among all 10 features, from the least to the most important feature. Generally, the $\nth{2}$ feature ``set\_max\_transition" is the least important one. We notice that features show very similar importance across different designs, especially for those unimportant features. This shows that transferring feature importance from prior data is reasonable. 

The similarity of samples by different sampling methods is shown in Table \ref{tbl:samp}. It compares random sampling, sampling within cluster,  and sampling from different clusters. The standard deviations $\sigma$ of their solution quality are measured. The ``true" and ``learn" in parentheses indicate whether feature importance is ground-truth or learned from other designs. The in-cluster sampling gives much lower $\sigma$, which verifies that samples from the same cluster have a much more similar design quality. This provides the rationale of using $\widetilde{S}_{approx}$ with approximate labels. The learned in-cluster $\sigma$ is only slightly higher than ground truth for timing, again indicating that learned feature importance is pretty close to truth. 

However, $\sigma$ for cross-cluster sampling is not much higher than random sampling. That means simply sampling from different clusters does not lead to more representative samples. That is also why approximate samples  $\widetilde{S}_{approx}$ are necessary in such clustering strategy. 



\begin{table}[!t]
  \centering
  \caption{Standard deviation of samples.}
  \label{tbl:samp}
  \resizebox{0.9\linewidth}{!}{%
  \begin{tabular}{l | c| c |c}
  \hline
                           & Power   & SetTime & HoldTime   \\
  \hline
    Random sampling         &  3.35  &   0.377  &  0.288    \\  
  \hline
   In-cluster sampling (learn)    &  0.49  &   0.152  &  0.175    \\
   Cross-cluster sampling (learn) &  3.42  &   0.384  &  0.282    \\
   \hline
   In-cluster sampling (true)    &  0.54  &   0.135  &  0.146    \\
   Cross-cluster sampling (true) &  3.39  &   0.383  &  0.294    \\
  \hline
  \end{tabular}
  }
\end{table}




\iffalse
\subsection{Tree-based Methods}

To study why random forest is inferior to XGBoost, influence of tree number in random forest is analyzed in Figure \ref{rf_trees}. Surprisingly, results are worse as number of trees increases. The best result is achieved when only one tree exists. At this time random forest degrades to a normal decision tree. 

A possible explanation is that random forest results in a too stable learning model because it largely reduces variance by averaging trees. This is a good property in general tasks, but can be harmful in space exploration. A recent study in DSE \cite{meng2016adaptive} proves almost half Pareto samples can be missed even for a well-trained model. As a result, a more stable learner decreases the probability of Pareto samples to be identified compared with a relaxed model. XGBoost, as a boosting tree model, performs much better since it mainly reduces bias.
\fi

%We look into the accuracy of models. Figure \ref{kendall} shows the Kendall rank correlation  \cite{kendall1938new} between prediction and ground-truth labels. A higher coefficient means a more accurate ranking. It also presents the standard deviation of Kendall coefficient calculated from 500 randomized trials in `P\_std', `ST\_std', `HT\_std'. The kendall coefficient and standard deviation partially reflect model accuracy and variance, respectively. Like we expected, Random Forest with more trees are more accurate but with less variance. 



%By ensemble of multiple trees, Random Forest reduces its variance without reducing bias. 

\iffalse
\begin{figure}[!t]
  \centering
%  \begin{minipage}[t]{3.5in}
    \includegraphics[width=\columnwidth]{RF_trees}
  \caption{Influence of tree number in random forest.}
  \label{rf_trees}
%  \end{minipage}
\end{figure}
\fi

\iffalse
\begin{figure}[!thb]
  \centering
  \begin{minipage}[t]{3.5in}
    \includegraphics[width=3.5in]{kendall}
  \caption{Accuracy and variance of methods}
  \label{kendall}
  \end{minipage}
\end{figure}
\fi
 
 %\begin{table}[!thb]



%\subsection{Dynamic Depth}
%There are two major reasons for dynamic depth strategy: 1. Flexibility of model is compatible with number of samples. 2. When tree depth is low, a more relaxed sampling method accepting more candidates is performed.

%There are two general strategies in space exploration process, exploration and exploitation. The prior one corresponds to modeless sampling and latter one corresponds to refinement sampling. But previous refinement methods perform a direct switch, which can miss many actual Pareto samples \cite{meng2016adaptive}. Thus, by setting tree depth to be low and increase it dynamically, it slowly switches from exploration state to exploitation state.
